HEX: Humanoid-Aligned Experts for Cross-Embodiment Whole-Body Manipulation

Humans achieve complex manipulation through coordinated whole-body control, whereas most Vision-Language-Action (VLA) models treat robot body parts largely independently, making high-DoF humanoid control challenging and often unstable. We present HEX, a state-centric framework for coordinated manipulation on full-sized bipedal humanoid robots. HEX introduces a humanoid-aligned universal state representation for scalable learning across heterogeneous embodiments, and incorporates a Mixture-of-Experts Unified Proprioceptive Predictor to model whole-body coordination and temporal motion dynamics from large-scale multi-embodiment trajectory data. To efficiently capture temporal visual context, HEX uses lightweight history tokens to summarize past observations, avoiding repeated encoding of historical images during inference. It further employs a residual-gated fusion mechanism with a flow-matching action head to adaptively integrate visual-language cues with proprioceptive dynamics for action generation. Experiments on real-world humanoid manipulation tasks show that HEX achieves state-of-the-art performance in task success rate and generalization, particularly in fast-reaction and long-horizon scenarios.

==> tables/few-shot_fine-tune.tex <==
\begin{table}[t]
\centering
\small
\caption{Few-shot fine-tuning results on the \emph{Basket transfer from bed to table} task using different fractions of the downstream training data.}
\label{tab:fewshot}
\vskip -0.05in
\begin{tabular}{c|cc}
\toprule
Fine-tuning Ratio & SR (\%) $\uparrow$ & SPS $\uparrow$ \\
\midrule
0\%   & --   & --    \\
10\%  & 0.0  & 0.00  \\
20\%  & 0.0  & 3.33  \\
50\%  & 0.0  & 19.44 \\
100\% & \textbf{86.6} & \textbf{91.67} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/metric.tex <==
\begin{table*}[htbp]
{\color{red}
\centering
\caption{Stage definitions and weights for computing the Stage-wise Progress Score (SPS) on four evaluated real-world tasks.}
\label{tab:stage_score}
\vskip -0.05in
\small

\makebox[\textwidth][c]{%
\begin{tabular}{
    >{\raggedright\arraybackslash}m{0.17\textwidth}
    >{\centering\arraybackslash}m{0.13\textwidth}
    >{\centering\arraybackslash}m{0.13\textwidth}
    >{\centering\arraybackslash}m{0.13\textwidth}
    >{\centering\arraybackslash}m{0.14\textwidth}
    >{\centering\arraybackslash}m{0.10\textwidth}
}
\toprule
\textbf{Task} &
\textbf{Stage 1} &
\textbf{Stage 2} &
\textbf{Stage 3} &
\textbf{Stage 4} &
\textbf{Stage 5} \\
\midrule

\makecell[l]{Basket transfer\\from bed to table} &
\makecell[c]{Pick up basket\\{\scriptsize ($w=3$)}} &
\makecell[c]{Turn around\\{\scriptsize ($w=2$)}} &
\makecell[c]{Walk to table\\{\scriptsize ($w=3$)}} &
\makecell[c]{Place basket\\{\scriptsize ($w=2$)}} &
-- \\

\makecell[l]{Toy transfer\\to cart basket} &
\makecell[c]{Pick up toy\\{\scriptsize ($w=3$)}} &
\makecell[c]{Turn around\\{\scriptsize ($w=2$)}} &
\makecell[c]{Walk to cart\\{\scriptsize ($w=4$)}} &
\makecell[c]{Place toy\\in basket\\{\scriptsize ($w=3$)}} &
-- \\

\makecell[l]{Pour liquor while\\following human order} &
\makecell[c]{Pick up container\\{\scriptsize ($w=3$)}} &
\makecell[c]{First cup\\{\scriptsize ($w=3$)}} &
\makecell[c]{Second cup\\{\scriptsize ($w=3$)}} &
\makecell[c]{Third cup\\{\scriptsize ($w=3$)}} &
\makecell[c]{Return arm\\{\scriptsize ($w=2$)}} \\

\makecell[l]{Long-horizon\\box convey} &
\makecell[c]{Pick up box\\{\scriptsize ($w=3$)}} &
\makecell[c]{Turn around\\{\scriptsize ($w=2$)}} &
\makecell[c]{Walk to table\\{\scriptsize ($w=4$)}} &
\makecell[c]{Place box\\{\scriptsize ($w=3$)}} &
-- \\

\bottomrule
\end{tabular}%
}
}
\end{table*}
